Target conversation extraction: Source separation using turn-taking dynamics

Extracting the speech of participants in a conversation amidst interfering speakers and noise presents a challenging problem. In this paper, we introduce the novel task of target conversation extraction, where the goal is to extract the audio of a target conversation based on the speaker embedding of one of its participants. To accomplish this, we propose leveraging temporal patterns inherent in human conversations, particularly turn-taking dynamics, which uniquely characterize speakers engaged in conversation and distinguish them from interfering speakers and noise. Using neural networks, we show the feasibility of our approach on English and Mandarin conversation datasets. In the presence of interfering speakers, our results show an 8.19 dB improvement in signal-to-noise ratio for 2-speaker conversations and a 7.92 dB improvement for 2-4-speaker conversations. Code, dataset available at https://github.com/chentuochao/Target-Conversation-Extraction.

==> method.tex <==
\section{Methods}
\subsection{Problem formulation}

Let $x(t) \in \mathbb{R}^T$ be the noisy conversation signal of length $T$. This signal can be decomposed as:
$$ 
 x = s_0 + \sum_{i=1}^N s_{i}^{conv} + \sum_{j=1}^M s_{j}^{inter} + n$$
Here, $s_0$ corresponds to the speech of the reference speaker in the conversation. $s_{1}^{\text{conv}},\ldots,s_{n}^{\text{conv}}$ are the other speakers  in  target conversation,  $s_{1}^{\text{inter}},\ldots,s_{m}^{\text{inter}}$ are the interfering speakers not part of the conversation, and $n$ is background noise. 


Given  an embedding for the  reference speaker,  ${\epsilon}_0 \in \mathbb{R}^D$ of length $D$, the goal of the target conversation extraction network, $\mathcal{N}$, is to extract the entire target conversation:
$$y = \mathcal{N}(x | \epsilon_0) =   \hat{s}_0 + \sum_{i=1}^{N} \hat{s}_i^{conv} $$
where,  $\hat{s}_0$ is an  estimate of $s_0$ and $\hat{s}_j^{conv}$ is an estimate of $s_j^{conv}$.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\linewidth]{figure/Arch.png}
  \caption{architecture}
  \label{fig:architecture}
\end{figure}

\subsection{Speaker embedding for reference speaker}

The intuition behind our neural network design is that the model can use the reference speaker embedding to identify their speech in the mixture and subsequently identify other target speakers in the conversation, by using the  turn-taking cues. % with the user's speech. %However, to achieve this goal, there are some technical challenges: (1)  (2) During training, we need to create the synthetic mixture from the spoken conversation dataset, however since the conversation speech are recorded with the same device and environment,  


\subsection{Network architecture}
The intuition behind neural network design is that the model can initially use a clean example to extract the user's speech and subsequently identify other target speakers by matching turn-taking cues with the user's speech. %However, to achieve this goal, there are some technical challenges: (1)  (2) During training, we need to create the synthetic mixture from the spoken conversation dataset, however since the conversation speech are recorded with the same device and environment,  

\textbf{Speaker embedding from clean example} A common way to extract speaker-related information from the speech example is the d-vector or i-vector~\cite{i_vector,d_vector}, which has been extensively adopted in the target speaker extraction task~\cite{speakerbeam}. In our work, we use the open-source implementation (Resemblyzer~\cite{Resemble-Ai}) of d-vector. It deploys a long short-term memory
(LSTM) network to extract a unit length 256-
dimensional vector $\epsilon^0 \in R^{256}$ from the clean example $e^0$. To condition our separation model with the user's speaker information (i.e., $\epsilon^0$), we apply the FilM layer~\cite{perez2018film} to merge the extracted speaker information and intermediate TF representation in the separation model. 

\textbf{Conversation extraction module}
Recently, a lot of universal source separation models have been proposed~\cite{xxx}. TF-GridNet~\cite{wang2023tf} is one of state of arts, that applies LSTM on both frequency dimension and time dimension, followed by a full-band self-attention module. It has shown advanced separation ability and strong robustness to noise and reverberation. Most of the source separation models focus on second-level audio separation (3-5 s)~\cite{xxx}. However, since we leverage the turn-taking cues of conversation for separation, the model should have a receptive field of the entire minute-level sequence. The recurrent network is not suitable for long sequences due to its Parallelization Difficulty and Limited Long-range Memory~\cite{vaswani2017attention, melis2017state}. Recently, people utilized attention modules ~\cite{vaswani2017attention} but it suffers from quadratic time complexity~\cite{fastformer, longformer}. To reduce the complexity of long sequences, many efficient and sparse Attention mechanisms are proposed, like Slide-window Attention~\cite{longformer}, Hashing Attention~\cite{reformer}, and Pooling Attention~\cite{poolingformer}. In the speech domain, RE-Sepformer, XNOR-former, and others \cite{resepformer, speechLongformer, xnorformer} explore the sparse attention on speech tasks. 

Inspired by these works, our model is shown in Fig.~\ref{xxx}. 
Firstly, we apply the short-time Fourier transform (STFT) to get TF representation of the mixture $X\in R^{T\times F}$.  Then we stack the real and imaginary parts and pass them to a 2D convolution with a 3 × 3 kernel to get $Y\in R^{D\times T \times F}$. $D$ is the embedding dimension for each TF grid. The $Y$ is passed to $B$ repeated extraction blocks conditioned by the speaker embedding. Finally, the processed TF representation is passed to a 2D deconvolution (3x3 kernel) and inverse STFT (iSTFT) to recover the time-domain speech.   

Each extraction block is composed of two modules: a local module and a global module. First, we apply a sliding window with $W$ window size and stride size $S$ on the $Y$ to get $Z_l \in R^{C \times D \times W \times F}$, where $C$ is the number of sliding windows. 
The local module is based on the TF-GridNet block~\cite{wang2023tf}  and applies to each sliding window individually. Specifically, we first apply a one-layer bidirectional long short-term memory (BLSTM) with hidden size $H$ on the frequency domain $F$, followed by a deconvolution layer with $2H$ input channels and $D$ output channels. After that, another one-layer bidirectional long short-term memory (BLSTM) with hidden size $H$ is applied on the time domain, and the sequence length is limited to $W$ due to the sliding window. Then it also passes to a deconvolution layer. 
The global module is designed to capture long-range global information (turn-taking cues) inspired by PoolingFormer~\cite{poolingformer} and RE-Sepfromer~\cite{resepformer}. We apply the pooling operation (the same window size $W$ and stride size $S$) to compress long sequence $T$ to $C$, $Z_g \in R^{D \times C \times F}$. We first apply the positional encoding on $Z_g$ because the order information for conversation turn-taking is very important. We apply three linear layers to merge the $D$ and $F$ dimensions to obtain key $K\in R^{C \times E}$, query $Q \in R^{C \times E}$ and value $V \in R^{C \times (DF/L)}$, where $E$ is the embedding dimension for $K$, $Q$ and $L$ is the head number. Finally, we apply the self-attention across the dimension $C$, followed by a feedforward layer, and add the output to the input tensor via a residual connection. 

\textbf{Time-preserving data augmentation} During training, we need to create the synthetic mixture from the spoken conversation dataset by mixing conversation with other interference conversation or speaker. However, since each conversation is recorded with the same device and environment, the speech within the conversation may share the same acoustic properties (like reverberations, background noise, and hardware distortion). In our preliminary experiments, we discovered that training the model by directly combining two conversation samples - even if they originate from the same dataset - leads the model to autonomously leverage acoustic properties for matching conversation speech, rather than relying on turn-taking cues, which would compromise the results. To address this issue and disentangle these acoustic properties, we propose a novel data augmentation and training methodology. Since we want to model to learn the timing cues, we can replace the speech of a speaker with the speech from a larger speech dataset (not necessarily a conversational dataset, such as LibriTTS) and preserve the original timing information. In particular, for each speaker in a conversation sample, with a probability of $p$, we randomly choose a new speaker from the larger speech dataset. Given that most conversational datasets provide timestamp labels, we can use the timestamp information to identify the spoken segment of the original speaker. Subsequently, we replace this segment with a randomly selected utterance with a similar length from the new speaker. Such augmentation can provide several benefits: (1) It disentangles the acoustic property and compels the model to learn the timing information (2) The introduction of larger non-conversational speech datasets significantly enhances speaker and speech diversity. (3) Since conversational audio is usually noisy (not originally designed for separation tasks), cleaner audio from larger datasets is better suited to serve as the ground truth for separation.

\textbf{Pretrain/Finetune} 
With the proposed Time-preserving data augmentation, we can create more conversational datasets from the non-conversational dataset to train the model. However, even if this augmentation can preserve timing information, other prosodic features such as pitch, voice quality, and intensity are removed and the spoken conversation becomes unnatural.  



When $p = 1$, we just replace all speakers with new speakers from a large dataset and we call it Synthetic Conversation (denoted by $\mathcal{S}$). When $p \in (0, 1)$, we partially replace the speakers and call it Augmented Conversation (denoted by $\mathcal{A}$). When $p = 0$, it is the original Real Conversation (denoted by $\mathcal{R}$).


